GAMEOPT+: Improving Fuel Efficiency in Unregulated Heterogeneous Traffic Intersections via Optimal Multi-agent Cooperative Control

Better fuel efficiency leads to better financial security as well as a cleaner environment. We propose a novel approach for improving fuel efficiency in unstructured and unregulated traffic environments. Existing intelligent transportation solutions for improving fuel efficiency, however, apply only to traffic intersections with sparse traffic or traffic where drivers obey the regulations, or both. We propose GameOpt+, a novel hybrid approach for cooperative intersection control in dynamic, multi-lane, unsignalized intersections. GameOpt+ is a hybrid solution that combines an auction mechanism and an optimization-based trajectory planner. It generates a priority entrance sequence for each agent and computes velocity controls in real-time, taking less than 10 milliseconds even in high-density traffic with over 10,000 vehicles per hour. Compared to fully optimization-based methods, it operates 100 times faster while ensuring fairness, safety, and efficiency. Tested on the SUMO simulator, our algorithm improves throughput by at least 25%, reduces the time to reach the goal by at least 70%, and decreases fuel consumption by 50% compared to auction-based and signaled approaches using traffic lights and stop signs. GameOpt+ is also unaffected by unbalanced traffic inflows, whereas some of the other baselines encountered a decrease in performance in unbalanced traffic inflow environments.

==> Sections/3C.tex <==
\subsection{\optname: Computing Optimal Velocities} 
\label{sec:optimization}

\noindent\textbf{The Optimization Problem:}

Based on the optimal priority sequence $q^*$ from Section~\ref{subsec: priority_order}, the optimal command velocities, $\bm{u}_i$, for each vehicle are computed by optimizing Equation~\ref{eq:opt_velocity} for a fixed sequence. We restate the objective function here for convenience:
%
\begin{equation}
\mathcal{J}(\bm{u}_i|q^*) = \min_{\{\bm{u}_i\}} \sum_{i=1}^n \lambda (\bm{u}_i-\bar v)^2 + (1-\lambda) (\bm{u}_i-v_i)^2
\label{eq:J}
\end{equation}
%

\noindent The first quadratic term of Equation~\ref{eq:J} prevents $\bm{u}_i$ from deviating from the speed limit  $\bar v$ (results in improved throughput). The second quadratic term minimizes the control effort applied to optimize fuel efficiency. Below we discuss constraints on safety and the influence of $q^*$ on Equation~(\ref{eq:J}).\\


\noindent \textbf{Constraints on Safety and Compliance with $\mathbf{q^*}$:} 

We consider both longitudinal (rear-end) collisions in the control zone and collisions in the conflict zone. Rear-end collisions along each of the lanes in the control zone are prevented by ensuring all vehicles in the same lane maintain a safe distance between each other. Formally,

\begin{equation} 
\Big | s_j^k(t+1)-s_{j\prime}^k(t+1)\Big | \geq l_{j} + M_{sr}
\label{eq: longitudinal_collision}
\end{equation}

\noindent for all $k$ lanes in the control zone and for all agents $j,j\prime$ with $j\neq j\prime$ in the $k^\textrm{th}$ lane. $l_j$ represents the length of the agent $j$ and $M_{sr}$ is a safety margin added to maintain a safe gap between vehicles and to account for imperfections in sensing and actuation. We compute the future position $s_i(t+1)$ using,

\begin{equation}
\label{eq:eq_cons_3_1}
    s_i(t+1) = s_i(t) - \Delta t \left (\frac{v_i(t)+\bm{u}_i(t)}{2}\right)
\end{equation}

\noindent Here, $\Delta t$ is defined as the planning time step of the controller.

Next, we also need to ensure that no collisions occur inside the conflict zone. This task reduces to ensuring no vehicles belonging to conflicting lane groups (\ref{subsec: conflict_resolution}) enter the intersection simultaneously. Therefore, for each vehicle $i$ in the sequence $q^*$, paired with a vehicle $j$ in a conflicting group where $i$ has higher priority over $j$, we add the constraint,

\begin{equation}
    % \begin{array}{c}
        t_c^i + \frac{(l_i + M_{sl})}{\bm{u}_i} \leq t_c^{j}
        % t_c^i \leq t_c^{j} - \frac{l^i}{\bm{u}_i} - \frac{l^{i+1}}{u_{i+1}} - M_{sl}
    % \end{array}
    \label{eq: lateral_collision}
\end{equation}
%

\noindent where $t_c^i= \frac{s_i(t+1)}{\bm{u}_i}$ represents the time at which $i$ would arrive at the intersection. The above constraint ensures that command velocities $\bm{u}_i$ are chosen such that vehicles proceed through the conflict zone in the order of the sequence under consideration $q^*$. Note that this constraint is applied to every conflicting pair of vehicles; non-conflicting vehicles are allowed to enter the intersection at the same time, increasing the efficiency of the system. The safety margin $M_{sl}$ corresponds to the width of the intersection and prevents lateral collisions occurring when conflicting vehicles cross the intersection. 

The safety constraints with respect to ordering $q^*$ in Equations~(\ref{eq: longitudinal_collision}) and~(\ref{eq: lateral_collision}) result in an intractable mixed-integer quadratic programming (MIQP) optimization problem. This problem is further compounded due to lane indexing, which introduces a new variable indicating the agent's lane. We remove the dependency over the lane index by separating the constraints for each lane and using the multi-lane conflict resolution scheme introduced in~\ref{subsec: conflict_resolution}. This results in simplification of Equations~(\ref{eq: longitudinal_collision}) and~(\ref{eq: lateral_collision}), reformulating the original MIQP as a quadratic programming (QP) optimization problem; this QP can be solved in real-time. More formally, Equation~(\ref{eq: longitudinal_collision}) can be simplified as,

\begin{equation}
\label{eq: long_linear}
    \begin{aligned}
        % \begin{array}{c}
        \bm{u}_{j}^k-\bm{u}_{j+1}^k \geq & \left(v_{j+1}^k-v_{j}^k\right) \\
        & + \frac{2}{\Delta t}\left(s_{j}^k-s_{j+1}^k+l_{j}+M_{sr}\right) 
        % \end{array}
    \end{aligned}
\end{equation}

\noindent for all $k$ lanes in the control zone and for all $j,j+1$ consecutive vehicles belonging to lane $k$. And Equation~(\ref{eq: lateral_collision}) can be simplified as,


\begin{equation}
\label{eq: lateral_linear}
    % \begin{array}{c}
        \bm{u}_{j}\left(s_i-\frac{\Delta t}{2}.v_i+l_i+M_{sl}\right) 
        \leq \bm{u}_i\left(s_{j}-\frac{\Delta t}{2}.v_{j}\right) 
    % \end{array}
\end{equation}
%
for all vehicles $i$ in sequence $q^*$ and for all vehicles $j$ in a conflicting group to vehicle $i$.

Finally, we enforce reachability by bounding the command velocities by the speed limit, $\bar v$, as well as the acceleration and breaking capabilities of each individual vehicle.

\begin{equation}
\label{eq:eq_cons_1}
    0\leq \bm{u}_i(t)\leq \bar v
\end{equation}
\begin{equation}
\label{eq:eq_cons_2}
    a^{min}_i \Delta t\leq \bm{u}_i(t)-v_i(t)\leq a^{max}_i \Delta t
\end{equation}

\noindent\textbf{Solving \optname:} \textit{The constraints (\ref{eq: long_linear}), (\ref{eq: lateral_linear}), (\ref{eq:eq_cons_1}), and (\ref{eq:eq_cons_2}) are provided to \optname with objective function given by Equation~(\ref{eq:J}), which is solved numerically using Gurobi (version 9.1.2) \cite{gurobi}.}

The computed target $\bm{u}_i$ command velocities are transmitted to each of the CAVs in the control zone. Note that we do not consider delays in communication and assume the data is transmitted instantaneously via V2I communication. The low-level controller on-board each CAV then computes the optimal acceleration or deceleration needed, to achieve the desired $\bm{u}_i$ command velocity within the control time ($\Delta t$) duration. 

Finally, a key feature of our approach is that it is robust to drift in the executed control. Our approach operates at a cycle frequency of $100$ ms after which new command velocities are obtained, updating the previous controls. Therefore, any deviation between optimal control and the executed control is erased during every $100$ ms update cycle.

% There may always be unforeseen changes to the vehicles environment at execution time. Therefore, the low-level vehicle controller should attempt to reach the target velocity only as long as it is safe to do so. The CAV can utilize its on-board sensors to check whether the target velocity is safely reachable by the CAV. Any such discrepancy between target control velocity and executed safe control will be picked up and adjusted for by the high level controller in the next planning time step.


% This low-level controller should be made robust enough to handle perturbations in both sensing and actuation, as these are often noisy in practical scenarios. There can always be certain failures in sensing and communication. 

% \subsection{Multi-lane Intersection planning and control }
% \label{subsec: conflict_resolution}

% A key ability of our method is its ability to handle traffic effectively in multi-lane intersections. The extension from single lane to multi-lane is not straight forward. Many assumptions that can be made in single lane (such as one vehicle at a time in conflict zone) do not hold up in a multi-lane scenario. Thereby we introduce a system of classifying all vehicles in the control zone into groups based on their origin road and lane in order to handle conflicts among vehicles accurately. Fig. \ref{fig: conflict_groups} shows the different trajectories that vehicles in each lane can take along with the labeling of each of the lanes in the intersection.

% \input{img/multi-lane-conflict}

% Here, we notice that vehicle taking right turns at the intersection (groups 0-0,1-0,2-0,3-0) do not conflict with any other vehicle groups. Therefore, they are allowed to enter into the intersection freely and the constraints in the optimization in \ref{sec:optimization}, reflect this. For each of the remaining lane groups we need to identify which other lane groups can be allowed to enter the intersection at the same time. We denote this collection as the non-conflicting group set for each corresponding main lane group as shown in Table \ref{table: grouping}. 
% %
% For example consider the main lane group 0-1 (from road 0 and moving straight). The groups that do not conflict with this main group are  0-2 (from road 0 and turning left), 1-1 (from road 1 and moving straight) and 2-2 (from road 2 and turning left) along with all the right turn groups (0-0,1-0,2-0,3-0).
% %
% What this effectively means is that any vehicles belonging to the non-conflicting group set of a main lane group will be allowed to enter the intersection at the same time along with a vehicle of the main lane group.


% Note that right turn at the intersection groups (0-0,1-0,2-0,3-0) are directly marked as non-conflicting, and are included in the non-conflicting groups list for all vehicle groups by default.


==> Sections/Theory.tex <==
\section{Analysis of different bidding strategies}
\label{sec: np-complete}
\input{Tables/comp_auctions}
\input{{Tables/accuracy}}

At this point, there are two concerns that may come to the mind of the reader:

\begin{enumerate}[noitemsep]
    \item Justification of using driver behavior as the bidding strategy as opposed to using monetary budgets, arrival times, or any random driver-specific property, \textit{e.g.} height.
    
    \item Since the optimal solution in \model~is to reward more aggressive drivers, conservative agents may be motivated to act aggressively.
\end{enumerate}

\noindent In the following, we formally address both issues.
% In Section~\ref{subsec: alternate_strat}, 

% we show that in economic auctions, random bidding (using arbitrary driver properties \textit{e.g.} height), and FIFO-based strategies, agents actually gain more utility by over-bidding implying that such auctions are not incentive-compatible whereas behavior-based bidding is game-theoretically optimal (Section~\ref{subsec: optimality}).

% In Section~\ref{subsec: behavior_and_conservative}, we provide an insight into why 

\subsection{Justifying behavior-based bidding for human drivers with social preferences}
\label{subsec: alternate_strat}

The key insight to achieving an optimal auction is that agents' bidding strategy ($\bm{b}$) should be correlated with their social preferences or private valuations ($\bm{v}$). That is,

\begin{equation}
\begin{split}
    \bm{b}_1 > \bm{b}_2& > \ldots > \bm{b}_K\\
    &\iff\\
    \bm{v}_1 > \bm{v}_2& > \ldots > \bm{v}_K\\
\end{split}
\end{equation}

\noindent \hllb{where $\iff$ denotes equivalency} and with optimality occurring when $\bm{b}_i = \bm{v}_i = \bm{\zeta}_i$. In the case of behavior-based bidding, we explicitly enforce the above constraints via \model. Economic auctions, random bidding, and FIFO-based strategies, on the other hand, disregard the aspect of human social preference ($\bm{v}$). A simple analysis reveals that ignoring private valuations can result in auctions where agents are encouraged to falsify their bids.

% As before, let $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ and $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$ denote the order of bids and associated time-rewards for agents $a_1, a_2, \ldots, a_K$. The nature of bids depend on the particular mechanism; they represent money in the case of economic auctions and time-to-intersection (or roundabout) in the case of FIFO-based auctions.
Consider any economic auction~\cite{carlino2013auction}. Let the cash bids made by agents be $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ with associated time rewards, $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$. Now assume a single agent $a_k$ is an impatient driver with a budget $B_k$ and bid $\bm{b}_k \leq B_k$ ($B_k < B_m$ where $m$ indexes those agents whose bid $\bm{b}_m > \bm{b}_k$). Since economic auctions do not take social preferences or private valuations into account, it can be shown that $\bm{v}_k > \bm{b}_k$ for the impatient agent $a_k$. To see how, recall that $a_k$'s private valuation $\bm{v}_k$ is much higher than the agents before them. That is, $\exists m<k$ such that $\bm{v}_k > \bm{v}_m$. Without loss of generality, assume $m=k-1$. Then we have that $\bm{v}_1 > \ldots>\bm{v}_k> \bm{v}_{k-1}>\ldots> \bm{v}_K$. Since $\bm{v}_k>\bm{v}_{k-1}$ but $\bm{b}_{k-1}>\bm{b}_k$ and $\bm{v}_{k-1} = \bm{b}_{k-1}$, $\bm{v}_k > \bm{b}_{k}$ and $a_k$ can decide to increase her bid to $\bm{\bar b}_k = \bm{b}_{k-1} + \epsilon >\bm{b}_{k-1}$. The updated utility for $a_k$ is,

\begin{equation*}
% \begin{split}
    \bm{\bar u}_k (\bm{\bar b}_k) = \bm{v}_k \left( \frac{1}{t_{k-1}} \right ) - \sum_{j=k-1}^K \bm{b}_{j+1} \left(\frac{1}{t_j} - \frac{1}{t_{j+1}} \right).
% \end{split}    
\end{equation*}

\noindent The difference from original utility is,

\begin{equation}
% \begin{split}
    % &\bar u_k (\bar \bm{b}_k) = \\
    \bm{d} = \left( \bm{v}_k - \bm{b}_k \right)  \left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}} \right ).
    \label{eq: difference}
% \end{split}    
\end{equation}
    

\noindent Since $\bm{v}_k > \bm{b}_k$ and $t_{k-1} < t_{k}$, the net change is positive. Therefore, agents gain utility by over-bidding. This implies that economic and FIFO-based auctions are not optimal. We present empirical evidence in Section~\ref{subsec: comparison_with_prior_methods}.


\subsection{Behavior-based bidding does not encourage conservative agents to act aggressively}
\label{subsec: behavior_and_conservative}
At first glance, it may seem that a similar argument can be made against our approach wherein it is biased towards aggressive drivers by rewarding them with higher priority, thereby encouraging conservative drivers to be more aggressive (over-bidding). However, this is not the case since in the case of behavior-based bidding, acting aggressively and therefore, over-bidding $\bm{b}_k > \bm{v}_k \implies \bm{d} < 0$ by Equation~\ref{eq: difference}. In other words, conservative drivers lose utility by acting aggressively. \hllg{This is because in the event of an overbid, the gain in time reward, $\bm{\zeta}_{k}\left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}}\right)$ is \textit{less} than the risk penalty, $\bm{b}_{k}\left( \frac{1}{t_{k-1}} - \frac{1}{t_{k}}\right)$. Special cases include when two or more agents decide to over bid at the same time. The driver behavior modeling algorithm, CMetric, automatically takes care of these issues as it outputs a real number ($\mathbb{R}$). In the unlikely event that the CMetric output for multiple vehicles be identical, we choose to break ties randomly.}


==> Sections/back.tex <==
\section{Background and Problem Formulation}
In this section, we begin by defining several key terms and stating the problem statement followed by the assumptions made in our approach. We briefly summarize the CMetric algorithm~\cite{cmetric} for behavior modeling and prediction and provide an overview on sponsored search auctions~\cite{roughgarden2016twenty}, which are widely used in game theory.

\subsection{Problem formulation}
\label{subsec: problem_formulation}

We frame navigating unsignaled intersections, roundabouts, and merging scenarios as a multi-agent game-theoretic non-sequential decision-making problem. We consider three unsignaled and uncontrolled traffic scenarios or environments -- intersections, merging, and roundabouts with multiple non-communicating human drivers and AVs. In each of the three scenarios, we refer to a traffic-agent as ``active'' if they participate in the decision-making process for navigating the scenario. For example, the lead traffic-agents in each service lane of a four-way intersection are active vehicles, while agents waiting in line behind their respective lead vehicle are non-active agents. We denote the active agents as a set $\mathcal{A} = \{a_1, a_2, \ldots a_n \}$. The action space for each active agent is a discrete set consisting of finite acceleration values. The state space consists of the position $x_t \in \mathcal{X}$ and velocity $v_t$ of each agent measured in a global coordinate frame (\textit{e.g.} GPS coordinates or $3-$D points obtained using GPS and lidars, respectively).

\subsection{Modeling human driver behavior}
\label{subsec: cmetric_background}

Each active agent is characterized by a behavior profile, $\bm{\zeta}_i$, which can be obtained via recent behavior modeling algorithms such as the SVO~\cite{schwarting2019social} and CMetric~\cite{cmetric}. In this work, we use CMetric to quantify the aggressiveness or conservativeness of a traffic-agent. This model provides an objective measure of aggressiveness based on driving maneuvers such as overspeeding, overtaking and so on. We briefly summarize the CMetric algorithm. To determine if an agent is aggressive or conservative, the algorithm begins by reading the trajectories of the ego-agent and surrounding vehicles via cameras or lidars during any time-period $\Delta t$. The trajectory of an agent is represented by 

\[\Xi_{\Delta t} = \{x_t \ | \ t = t_0, t_1, \ldots, t_0 + \Delta t \}.\]

\noindent In CMetric, these trajectories are represented via weighted undirected graphs $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ in which the vertices denote the positions for each agent and the edges correspond to the distances between agents. The algorithm proceeds by using these graphs to model the likelihood and intensity of driving behavior indicators like overspeeding, overtaking, sudden ``zig-zagging'' and lane-changes via centrality functions~\cite{rodrigues2019network} represented by $\Phi: \mathcal{G}\rightarrow \mathbb{R}$. These behavior indicators determine whether an agent is aggressive or conservative~\cite{sagberg2015review}. The behavior profile for $a_i$ is denoted by $\bm{\zeta}_i$ and can be computed using,

\begin{equation}
    \bm{\zeta}_i(\Xi_{\Delta t}) = \Phi(\mathcal{G}),
    \label{eq: cmetric}
\end{equation}

\noindent where $\mathcal{G}(\mathcal{V}, \mathcal{E})$ is constructed using $\Xi_{\Delta t}$. In this work, we use CMetric to compute the behavior profiles of traffic-agents, represented by a $n-$dimensional vector $\bm{\zeta},$ that is provided to the auction program.

\subsection{Assumptions}
\label{subsec: assumptions}

We assume agents (AVs and human drivers) are rational and strive to maximize their own utility which can be independent of other agents. Further, agents are \textit{non-ideal} (in contrast to ideal agents in~\cite{cleac2020lucidgames, cleac2019algames, wang2020game}) in that they do not have access to the actions, objectives, or utility functions of other agents. We make no assumptions on the motion or dynamics of traffic-agents. The state-space is fully observable by all agents (active and non-active). We assume the availability of a behavior modeling and prediction algorithm such as CMetric~\cite{cmetric} that models driving behavior as being either aggressive or conservative. This information is provided to an auction program. We assume that agents navigate through the environment one at a time and do not use traffic signals, employ right-of-way rules, or communicate with other agents.

\subsection{Sponsored search auctions (SSAs)}
\label{subsec: SSA_background}
Sponsored search auctions (SSAs) are a game-theoretic mechanism that are used extensively in internet search engines for the purpose of internet advertising~\cite{roughgarden2016twenty}. In an SSA, there are $K$ items to be allocated among $n$ agents. Each agent $a_i$ has a private valuation $\bm{v}_i$ and submits a bid $\bm{b}_i$ to receive at most one item of value $\bm{\alpha}_i$. A strategy is defined as an $n$ dimensional vector, $\bm{b} = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. $\bm{b}_{-i})$ denotes the bids made by all agents except $a_i$. Furthermore, let $\bm{b}_1 > \bm{b}_2 > \ldots > \bm{b}_K$ and $\bm{\alpha}_1 > \bm{\alpha}_2 > \ldots > \bm{\alpha}_K$. The allocation rule is that the agent with the $i^\textrm{th}$ highest bid is allocated the $i^\textrm{th}$ most valuable item, $\bm{\alpha}_i$. The utility $\bm{u}_i$~\cite{roughgarden2016twenty} incurred by $a_i$ is given as follows,

\begin{equation}
 \bm{u}_i (\bm{b}_i) =  \bm{v}_i \bm{\alpha}_i - \sum_{j=i}^k \bm{b}_{j+1} \left( \bm{\alpha}_j - \bm{\alpha}_{j+1} \right).
 \label{eq: utility_template}
\end{equation}

\noindent In the equation above, the quantity on the left represents the total utility for $a_i$ which is equal to value of the allocated goods $\bm{\alpha}_i$ minus a payment term. The first term on the right is the value of the item obtained by $a_i$. The second term on the right is the payment made by $a_i$ as a function of bids $\bm{b}_{j > i}$ and their allocated item values $\bm{\alpha}_j$. We refer the reader to Chapter $3$ in~\cite{roughgarden2016twenty} for a derivation and detailed analysis of Equation~\ref{eq: utility_template}.

In our approach, we re-cast Equation~\ref{eq: utility_template} through the lens of a human driver. More specifically, the term $\bm{v}_i \bm{\alpha}_i$ denotes the time reward gained by driver $a_i$ by moving on her turn. The payment term represents a notion of risk~\cite{wang2020game} associated with moving on that turn. It follows that an allocation of a conservative agent to a later turn (smaller $\bm{\alpha}$) also presents the lowest risk and vice-versa.

\subsection{Problem statement}

To prevent collisions and deadlocks, it is necessary to determine the order in which agents take turns to navigate the traffic scenario~\cite{carlino2013auction, dresner2008multiagent, lin2021pay, sayin2018information, schepperle2007agent, vasirani2012market}. Thus, the goal of this paper (formalized shortly via Problem~\ref{problem: prob}) is to compute an optimal turn-based ordering which is defined as follows,

% \input{NeuRIPS2020/img/overview/overview}

\begin{definition}
\textbf{Turn-based Orderings ($\bm{\sigma}$): } A turn-based ordering is a permutation $\bm{\sigma}: \mathcal{A} \rightarrow [1,n]$ over the set $\mathcal{A}$. For any $i,j \in [1,n]$, $\bm{\sigma}(a_i) = j$, equivalently $\bm{\sigma}_i = j$, indicates that $a_i$ with driving behavior $\bm{\zeta}_i$ will move on the $j^\textrm{th}$ turn.
\label{def: turn_based_ordering}
\end{definition}


\noindent There may be multiple turn-based orderings that may apply in a given scenario. However, many of them could be sub-optimal and may result in collisions and deadlocks. An optimal turn-based ordering prevents collisions and resolves deadlock conflicts.

\begin{definition}
\textbf{Optimal Turn-based Ordering ($\bm{\sigma}_{\textsc{opt}}$): } A turn-based ordering, $\bm{\sigma}$, over a given set $\mathcal{A}$ is game-theoretically optimal if it is incentive compatible, welfare maximizing, and can be computed in polynomial time\footnote{These terms are defined in Section~\ref{subsec: optimality}}.
\label{def: optimal_turn_based_ordering}
\end{definition}

\noindent We now ready to formally state our goal in this paper as follows,

\begin{problem}
In a traffic scenario (which could be an intersection, roundabout, or merging) with $n$ active road-agents, given the behavior profile $\bm{\zeta}_i$ of each agent, the goal is to compute the optimal turn-based ordering $\bm{\sigma}_\textsc{opt}  = \bm{\sigma}_1\bm{\sigma}_2\ldots\bm{\sigma}_n$.
\label{problem: prob}
\end{problem}


% \input{NeuRIPS2020/img/overview/overview}
% In game theory, a strategy is defined as an $n$ dimensional vector, $b = (\bm{b}_i \cup \bm{b}_{-i})$, representing the bids made by every agent. The goal of any optimal auction is to generate maximum welfare upon truthful bidding so that that no agent is incentivised to ``cheat'' \textit{i.e.} incentive compatible. In other words, auctions are incentive compatible when the dominant strategy for each agent is to bid their true valuation $v_i$.
% In our proposed approach, we combine the SSA with the CMetric behavior modeling algorithm to generate an auction with a novel bidding strategy. We discuss this approach in detail in the following section. 
% We conclude current section with the some standard, but important, definitions related to game-theoretic optimality.

% \begin{definition}
% \textbf{Dominant Strategy:} Bidding $\bm{b}_i$ is a dominant strategy for $a_i$ if $\bm{u}_i(\bm{b}_i, \bar \bm{b}_{-i}) > \bm{u}_i(\bar \bm{b}_i, \bar \bm{b}_{-i})$ for all $\bar \bm{b}_i \neq \bm{b}_i$.
% \end{definition}

% We now state two important definitions that are used as the basis of an optimal SSA.

% \begin{definition}
% \textbf{Incentive Compatibility:} An auction is said to be incentive compatible if for each agent, bidding $\bm{b}_i = v_i$ is a dominant strategy.
% \label{def: incentive_compatibility}
% \end{definition}

% \begin{definition}
% \textbf{Welfare Maximization:} Social welfare of an auction outcome is defined as $\sum_i v_i \bm{u}_i(\bm{b}_i)$. Welfare maximization is the task of finding the strategy $b$ that maximizes $\sum_i v_i \bm{u}_i(\bm{b}_i)$.
% \label{def: social_welfare}
% \end{definition}

% Finally, SSAs have polynomial time complexity since sorting is polynomial time~\cite{clrs}.
% \subsubsection{Sponsored Search Auctions}

% \subsubsection{Optimality and Efficiency of SSAs}




==> Tables/accuracy.tex <==
\begin{table}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\caption{\textbf{Comparing with other approaches:} We compare the percentage \hllb{(\%)} of collisions (C), deadlocks (D), and overall success rate (S) with state-of-the-art planning methods designed for uncontrolled and unsignaled intersections. The \xmark~symbol indicates that results for that setting were not provided by the method.
}
\centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
\resizebox{\columnwidth}{!}{
\begin{tabular}{rccccccccc}
  \toprule[1.5pt]
%   \multirow{4}[3]{*}{Methods}&&&&$4-$way intersection&&&&&\\ 
%   \cmidrule[1pt](l{3mm}r{3mm}){3-13}   &
% \midrule
 \multirow{2}{*}{Methods}& \multicolumn{3}{c}{$2$ Vehicles} &
  \multicolumn{3}{c}{$3$ Vehicles}&  
  \multicolumn{3}{c}{$4$ Vehicles}\\
%   \cmidrule{3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
   & {C } & {D } & S  &  {C } & {D } & S  &  {C } & {D } & S \\
%   \midrule
%   \midrule
\midrule
%  &&&&&&$4-$way Intersection Groups&&&&&&\\ 
%   \midrule

  Capasso et al.~\cite{capasso2021end} & 
    \xmark & \xmark & \xmark & 
    $02$ & \xmark & \xmark & 
    $0$ & \xmark & \xmark  \\ 
  Liu et al.~\cite{liu2020decision} & 
    \xmark & \xmark & \xmark & 
    \xmark & \xmark & \xmark & 
    $6.2$ & \xmark & $93.7$  \\ 
  Isele et al.~\cite{isele2018navigating} & 
    \xmark & \xmark & \xmark & 
    \xmark & \xmark & \xmark & 
    $7.1$ & $0.2$ & $92.8$  \\ 
Kai et al.~\cite{Kai2020AMR} & 
    $0$ & $0$ & $100$ & 
    \xmark & \xmark & \xmark & 
    $3.7$ & $0 $ & $96.3$  \\ 
    
  Li et al.~\cite{li2020game} & 
    $0$ & $0$ & $100$ & 
    \xmark & \xmark & \xmark & 
    $2.7$ & $0.4$ & $96.9$  \\ 
  Roh et al.~\cite{roh2020multimodal} &
    $2$ & \xmark & $98$& $2$ & \xmark & $98$ & $30$ & \xmark & $70$   \\ 
  Tian et al.~\cite{tian2020game} &
    $10$ & $5$ & $85$ & 
    $10$ & $5$ & $85$ & 
    $10$ & $10$ & $80$  \\ 
  \model  & 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ & 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ & 
    $\textbf{0.1}$ & $\textbf{0.1}$ & $\textbf{99.8}$  \\ 
  \midrule
  
%  \midrule
%   \midrule
%     \multirow{4}[3]{*}{Methods}&&&&$ 4-$way intersection&&&&&\\ 
%   \midrule
  \multirow{2}{*}{Methods}&
  \multicolumn{3}{c}{$6$ Vehicles}& 
  \multicolumn{3}{c}{$8$ Vehicles}&  
  \multicolumn{3}{c}{$10$ Vehicles}\\
%   \cmidrule(l{3mm}r{3mm}){3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
   & {C } & {D } & S  &  {C } & {D } & S  &  {C } & {D } & S \\
  \midrule
    Capasso et al.~\cite{capasso2021end} & 
    \xmark & \xmark & \xmark &
    $03$ & \xmark & \xmark &
    \xmark & \xmark & \xmark  \\
  Li et al.~\cite{li2020game} &
    $10$ & $10$ & $90$ &
    $20$ & $20$ & $80$ &
    $20$ & $20$ & $80$  \\ 
  Tian et al.~\cite{tian2020game} &
    $10$ & $10$ & $80$ &
    $10$ & $10$ & $80$ &
    $20$ & $20$ & $60$  \\ 
    
    \midrule
  \model  &
    $\textbf{0.3}$ & $\textbf{0.1}$ & $\textbf{99.6}$ &
    $\textbf{0.4}$ & $\textbf{0.1}$ & $\textbf{99.5}$ &
    $\textbf{0.6}$ & $\textbf{0.2}$ & $\textbf{99.2}$  \\ 


  \bottomrule[1.5pt]
\end{tabular}
}
% \end{adjustbox}
% \vspace{-6mm}
\label{tab: accuracy}
  \vspace{-10pt}
 
\end{table}

==> Tables/benefits.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Benefits of \model~over prior work in planning.}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}

\toprule
%  &  &  & \multicolumn{2}{c}{Our CMetric Measures}\\

% \cline{4-5}
Problem Setting & Approach & Methods & Assumptions/Limitations & Benefits\\
\midrule
\multirow{2}{*}{Single-agent planning with dynamic obstacles} & Geometric Methods  && \\
                                             & Learning-based Methods && \\


\multirow{2}{*}{Multi-agent planning} & Game theory  && \\
                                             & Auctions && \\
 
\bottomrule
\end{tabular}
}
\label{tab: benefits}

\end{table*}

==> Tables/bidding.tex <==
\begin{table}%[tbhp]
\centering
\caption{\textbf{Summary of prior work:} We list methods for navigating unsignaled intersections, roundabouts, and merging based on multi-agent planning (MAP), action space (AS), and incentive compatibility (IC). \cmark$^{*}$ corresponding to a method indicates that optimality does not hold for human drivers with varying social preferences.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrccccc}
\toprule
Approach & Methods & Optimality & Multi-Agent & Planner & Cost & Dynamic\\
\midrule
\multirow{4}{*}{\small DRL}& Capasso et al.~\cite{capasso2021end} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark &C & -& \cellcolor{red!25} \xmark\\
& Isele et al.~\cite{isele2018navigating} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&D & -& \cellcolor{red!25} \xmark\\
& Kai et al.~\cite{Kai2020AMR} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark& D & -& \cellcolor{green!25} \cmark\\
& Liu et al.~\cite{liu2020decision} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&D & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

\multirow{2}{*}{\small Game Theory}& Li et al.~\cite{li2020game} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&C & -& \cellcolor{red!25} \xmark\\
& Tian et al.~\cite{tian2020game} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&C & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

{RNN} & Roh et al.~\cite{roh2020multimodal} &\cellcolor{red!25} \xmark&\cellcolor{red!25} \xmark&C & -& \cellcolor{red!25} \xmark\\
\cmidrule{2-7}

% \multirow{2}{*}{\small FIFO}& FIFO (basic) &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
% & Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
% \cmidrule{2-8}

\multirow{8}{*}{\small Auctions}& FIFO &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Vasirani and Ossowski~\cite{vasirani2012market}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Censi et al.~\cite{censi2019today}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Lin and Jabari~\cite{lin2021pay}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\
& Carlino et al.~\cite{carlino2013auction} &\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{red!25} \xmark\\
& Rey et al.~\cite{rey2021online}&\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{green!25} \cmark\\
& Sayin et al.~\cite{sayin2018information} &\cellcolor{green!25} \cmark$^{*}$&\cellcolor{green!25} \cmark&D & \cellcolor{green!25} \cmark& \cellcolor{red!25} \xmark\\
& Chandra and Manocha~\cite{chandra2022gameplan} &\cellcolor{green!25} \cmark&\cellcolor{green!25} \cmark&High & \cellcolor{green!25} \cmark & \cellcolor{red!25} \xmark\\
\cmidrule{2-7}
& \textbf{This work} &\cellcolor{green!25} \cmark&\cellcolor{green!25} \cmark&Hybrid & \cellcolor{green!25} \cmark & \cellcolor{green!25} \cmark\\

\multirow{1}{*}{\small Optimization}& Suriyarachchi et al.~\cite{suriyarachchi2021real} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Buckman et al.~\cite{gt6} &\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & -& \cellcolor{red!25} \xmark\\
& Vasirani and Ossowski~\cite{vasirani2012market}&\cellcolor{red!25} \xmark&\cellcolor{green!25} \cmark&D & \cellcolor{red!25} \xmark& \cellcolor{red!25} \xmark\\



\bottomrule
\end{tabular}
}
\label{tab: bidding_rules}
\vspace{-10pt}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}

\input{Tables/high_vs_low}

==> Tables/comp_auctions.tex <==
\begin{table*}[t]
{\fontsize{9pt}{9pt}\selectfont
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\caption{\textbf{Using different bidding strategies:} We compare the rate of collisions by replacing the CMetric bidding strategy with economic auctions, first-in-first-out (FIFO), and random bidding in a range of simulation settings that include changing the traffic density, number of aggressive drivers, likelihood of a driver being aggressive, and speed limit.}
\label{tab: auctions}
\centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
\fontsize{8}{10}\selectfont{\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccc|cc|cccc|cc@{}}
  \toprule
%   \multirow{4}[2]{*}{Methods}&&&&&&$4-$way Intersection&&&&&&\\ 
%   \cmidrule[1pt](l{3mm}r{3mm}){3-17
%   } 
  \multirow{2}{*}{Strategy} &
  \multicolumn{4}{c}{\% Aggressive}&
  \multicolumn{2}{c}{\# Agg. Agents}& 
  \multicolumn{4}{c}{\# Agents \fontsize{7}{8}\selectfont{(w. 1 agg. agent)}} & 
  \multicolumn{2}{c}{Max. Speed} \\
  \cmidrule{2-5} 
  \cmidrule{6-7} 
  \cmidrule{8-11}
  \cmidrule{12-13}
   & $20\%$ & $25\%$ & $33\%$ & $50\%$ &  $1$ & $2$  &  $4$ & $6$ & $8$ & $10$ & $45$mph & $60$mph \\
%   \midrule
%   \midrule
\midrule
%  &&&&&&$4-$way Intersection Groups&&&&&&\\ 
%   \midrule

  Economic & 
    $2.48$ & $2.99$ & $6.55$ &
    $8.29$& $2.81$ & $6.18$ & 
    $3.07$ & $3.27$ & $3.58$ & $3.62$ &$2.99$& $3.07$ \\ 
  FIFO & 
    $7.18$ & $8.69$ & $10.20$ & 
    $15.87$& $7.65$ & $15.06$ & 
    $7.59$ & $8.36$ & $8.65$ & $8.91$ & $7.72$ & $7.47$ \\ 
  Random  & 
    $14.79$ & $18.67$ & $25.24$ &
    $37.77$ & $15.01$ & $28.91$ & 
    $14.82$ & $16.69$ & $17.59$  & $17.90$& $15.01$&$15.01$\\ 
  \textbf{\model}  & 
     $\textbf{0.33}$ & $\textbf{0.37}$ & $\textbf{0.63}$ & 
    $\textbf{0.79}$& $\textbf{0.29}$ & $\textbf{0.66}$ & 
    $\textbf{0.12}$ & $\textbf{0.24}$ & $\textbf{0.37}$  & $\textbf{0.64}$& $\textbf{0.44}$&$\textbf{0.53}$\\ 

  \bottomrule
\end{tabular}}
}
}
% \end{adjustbox}
% \vspace{-6mm}
  \vspace{-5pt}
\end{table*}

==> Tables/high_vs_low.tex <==
\begin{table}[t]
    \centering
    \resizebox{.9\columnwidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule[1.25pt ]
        Approach & Intersection & \multicolumn{3}{c}{Optimality} & Realtime\\
        \midrule
          &  &  Safety & Efficiency & Fairness &\\
          \cmidrule{ 3-5}
          Auctions& \cellcolor{red!25} Static & \cellcolor{red!25} \xmark & \cellcolor{red!25} \xmark & \cellcolor{green!25} \cmark &\cellcolor{green!25} \cmark\\
          Game Theory & \cellcolor{green!25} Dynamic & \cellcolor{red!25} \xmark & \cellcolor{red!25} \xmark & \cellcolor{green!25} \cmark &\cellcolor{red!25} \xmark\\
          Optimization & \cellcolor{green!25} Dynamic & \cellcolor{green!25} \cmark & \cellcolor{green!25} \cmark & \cellcolor{red!25} \xmark &\cellcolor{red!25} \xmark\\
          Deep Learning & \cellcolor{red!25} Static & \cellcolor{red!25} \xmark & \cellcolor{green!25} \cmark & \cellcolor{red!25} \xmark &\cellcolor{green!25} \cmark\\
          \midrule
        \textbf{This work} & \cellcolor{green!25} Dynamic & \cellcolor{green!25} \cmark & \cellcolor{green!25} \cmark & \cellcolor{green!25} \cmark &\cellcolor{green!25} \cmark \\

          \bottomrule[1.25pt ]
    \end{tabular}
        }
    \caption{\textbf{Comparison with prior work:} We highlight approaches for navigating unsignalized intersections based on the type of intersection, optimality guarantees, and real-time capability.}
    \label{tab: comparison_table}
    \vspace{-10pt}
\end{table}

==> Tables/notation.tex <==
\begin{table}[t]
  \caption{Symbols and notations used in this paper.}
  \label{tab: notation}
  \centering
  \resizebox{.7\columnwidth}{!}{%
  \begin{wraptable}{r}{5.5cm}
  \begin{tabular}{cl}
  \toprule
    Symbol  & Description \\
    \midrule
    $n$ & Number of traffic-agents.\\
    $a_i$ & $i^\textrm{th}$ active agent.\\
    $\mathcal{A}$ & Set of active agents. \\
    $\zeta$ & CMetric-based behavior profile (Section~\ref{subsec: cmetric_background}). \\
    $\sigma$ & Turn-based ordering (Definition~\ref{def: turn_based_ordering}). \\
    $\sigma_{\textsc{opt}}$ & Optimal turn-based ordering (Definition~\ref{def: optimal_turn_based_ordering}). \\
    $b_i$ & Bid of the $i^\textrm{th}$ active agent.\\
    $b_{-i}$ & Bid of every agent except the $i^\textrm{th}$.\\
    $v_i$ & Private valuation of the $i^\textrm{th}$ active agent.\\
    $u_i(\cdot)$ & Utility of the $i^\textrm{th}$ active agent.\\
    $t_i$ & Time taken by the $i^\textrm{th}$ active agent \\
    & to navigate the traffic scenario.\\

    \bottomrule
  \end{tabular}
  \end{wraptable} 
  }
%   }
  \vspace{-15pt}
\end{table}


==> Tables/parameters.tex <==
\begin{table}[h]
\caption{IDM and MOBIL parameters used for Conservative and Aggressive vehicle classes}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clcc} 
\toprule
Model & Parameter \Tstrut & Conservative \Bstrut &   Aggressive \\
\hline
\multirow{4}{*}{IDM}& Time gap ( $T$) \Tstrut & 1.5s      & 1.2s \\
 &Min distance ($s_0$) & 5.0 $m$ & 2.5 $m$ \\
&Max comfort acc. ($a$)     & 3.0 $m/s^2$ & 6.0 $m/s^2$\\
&Max comfort dec. ($b$) & 6.0 $m/s^2$               &  9.0 $m/s^2$ \\
\midrule
\multirow{3}{*}{MOBIL}& Politeness ($p$) & 0.5     & 0\\
& Min acc gain ($\Delta a_{th}$) & 0.2 $m/s^2$ & 0 $m/s^2$ \\
& Safe acc limit ($b_{safe}$) & 3.0 $m/s^2$ & 9.0 $m/s^2$\\
\bottomrule
\end{tabular}
}
\label{tab: parameters}
\vspace{-10pt}
\end{table}


==> img/main_results.tex <==
\begin{figure*}[t]
\centering
   \begin{subfigure}[h]{0.325\textwidth}
    \includegraphics[width=\textwidth]{img/Throughput.png}
    \caption{Throughput}
    \label{fig: Throughput}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.325\textwidth}
    \includegraphics[width=\textwidth]{img/Time_spent.png}
    \caption{Time-to-goal}
    \label{fig: ttg}
  \end{subfigure}
    %
 \begin{subfigure}[h]{0.325\textwidth}
    \includegraphics[width=\textwidth]{img/Fuel_consumption.png}
    \caption{Fuel Efficiency}
    \label{fig: fuel_efficiency}
  \end{subfigure}

\caption{\textbf{Comparison with baselines:} \model increases throughput by approximately $25\%$ and $174\%$ compared to \textsc{Traffic-Light} and \textsc{Auction}, respectively. Furthermore, our method reduces the time-to-goal by $75\%$ and $81\%$, respectively, and improves fuel efficiency by $33\%$ and $66\%$, respectively, compared with \textsc{Traffic-Light} and \textsc{Auction}.
}
  \label{fig: results}
  \vspace{-15pt}
\end{figure*}             


